ULTRA: Unleash LLMs' Potential for Event Argument Extraction through Hierarchical Modeling and Pair-wise Self-Refinement

Structural extraction of events within discourse is critical since it avails a deeper understanding of communication patterns and behavior trends. Event argument extraction (EAE), at the core of event-centric understanding, is the task of identifying role-specific text spans (i.e., arguments) for a given event. Document-level EAE (DocEAE) focuses on arguments that are scattered across an entire document. In this work, we explore open-source Large Language Models (LLMs) for DocEAE, and propose ULTRA, a hierarchical framework that extracts event arguments more cost-effectively. Further, it alleviates the positional bias issue intrinsic to LLMs. ULTRA sequentially reads text chunks of a document to generate a candidate argument set, upon which non-pertinent candidates are dropped through self-refinement. We introduce LEAFER to address the challenge LLMs face in locating the exact boundary of an argument. ULTRA outperforms strong baselines, including strong supervised models and ChatGPT, by 9.8% when evaluated by Exact Match (EM).

==> tables/table_results_small.tex <==
\begin{table}[t]
\vspace{-3mm}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{llrrrr}
\toprule

\multicolumn{1}{c}{\multirow{2}{*}{Category}} & \multicolumn{1}{c}{\multirow{2}{*}{Method}}     & \multicolumn{2}{c}{Performance}                                                                                                                 & \multicolumn{2}{c}{Cost}                               \\ \cmidrule(lr){3-4}    \cmidrule(lr){5-6} 
                          &                                           & EM                                             & HM                                                 & Training & Inference \\ \midrule
\multirow{2}{*}{Supervised ML}                & EEQA* \citep{du-cardie-2020-event}          & 24.0                   & 55.5                   & \multirow{2}{*}{\$\$\$}      & \multirow{2}{*}{$\sim$0}   \\
                                              & Onology QA* \citep{tong-etal-2022-docee}    & 29.8                   & 56.9                   &                           &                            \\ \midrule
\multirow{3}{*}{Closed LLM}                & ChatGPT \citep{Li2023EvaluatingCI}        & 23.9                   & 65.2                   & \multirow{3}{*}{0}  & \multirow{3}{*}{\$-\$\$}        \\
                                              & ChatGPT (single question)                & 26.2                  & 64.4                   &                           &                            \\
                                              & CoT-ChatGPT \citep{wang-etal-2023-element}& 21.3                       & 62.1                   &                           &                            \\ \midrule
\multirow{2}{*}{Flan-UL2}                     & Custom instructions**                                        & 21.6                & 54.6                   & \multirow{2}{*}{\$}  & \multirow{2}{*}{$\sim$0}        \\
                                              & Aligned instruction                                & 26.3                  & 62.0                   &                           &                            \\
                                               \midrule
\multirow{4}{*}{\model (Ours)} & \model-base                                  & 31.5                   & 65.8                   & \multirow{4}{*}{\$}  & \multirow{4}{*}{$\sim$0}        \\
                                              & \; + Ensemble                    & \textbf{32.7}         & 69.0                   &                           &                            \\
                                              & \model-long                             & 31.4                    & 67.1                   &                           &                            \\
                                              & \; + Ensemble                   & 32.6         & \textbf{70.1}          &                           &                           \\ \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{F1 results on DocEE dataset for document-level event argument extraction. Breakdown of EM and HM scores by precision, recall and F1 are included in ~\Cref{tbl:results}. We also report estimated monetary cost by model category, divided into training and inference costs (\Cref{sec:cost_estimate}). Best results are shown in \textbf{bold}. \model achieves the best F1 performances at a reduced cost.  
The ablation study results of \model can be found in Table~\ref{tbl:results_additional}. *Results are taken from \citet{tong-etal-2022-docee}. **Average results of 5 instructions, results of individual custom instructions are included in Table~\ref{tbl:custom_results}.
} 
\vspace{-6mm}
\label{tbl:results_final}
\end{table}
